Document Context Language Models

Text documents are structured on multiple levels of detail: individual words are related by syntax, but larger units of text are related by discourse structure. Existing language models generally fail to account for discourse structure, but it is crucial if we are to have language models that reward coherence and generate coherent texts. We present and empirically evaluate a set of multi-level recurrent neural network language models, called Document-Context Language Models (DCLM), which incorporate contextual information both within and beyond the sentence. In comparison with word-level recurrent neural network language models, the DCLM models obtain slightly better predictive likelihoods, and considerably better assessments of document coherence.

==> tab-generation.tex <==

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

\begin{table}
  \centering
  \begin{tabular}{lp{11cm}}
    \toprule
    Context & Government officials here and in other countries laid plans through the weekend to head off a Monday market UNK -- but went out of their way to keep their moves quiet . Federal Reserve Chairman Alan Greenspan was on the UNK , making it clear to officials in the U.S. and abroad that the Fed was prepared to UNK massive amounts of money into the banking system , as it did in October 1987 , if the action were needed to prevent a financial crisis . And at the Treasury , Secretary Nicholas Brady talked with friends and associates on Wall Street while Assistant Secretary David UNK carefully UNK data on the Friday market plunge . \\
    Original & But the officials feared that any public announcements would only increase market jitters .\\
    Generation I & but UNK around at least the company 's responsibility for the Corporate paper 's performance . \\
    Generation II & so I cut concessions and concentrated ease .\\
    \midrule
    Context & The first major event this morning in U.S. stock and futures trading may be a UNK at the Chicago Mercantile Exchange . Under a reform UNK from the 1987 crash , trading in the Merc 's stock-index futures will break for 10 minutes if the contract opens and stays five points from Friday 's close , a move equal to 40 points on the Dow Jones Industrial Average . The aim of the UNK would be to ease the opening of the New York Stock Exchange , which would be UNK by such a volatile move on the Merc . That UNK UNK is just one of a number of UNK adopted after the 1987 crash . The Big Board also added computer capacity to handle huge UNK in trading volume . Several of those UNK changes kicked in during Friday 's one-hour collapse and worked as expected , even though they did n't prevent a stunning plunge . \\
    Original & But the major `` circuit breakers '' have yet to be UNK . \\
    Generation I & but analysts would not realize they expect to block money to seem UNK stations to understand fell to the UNK during UNK within the past . \\
    Generation II & so it was further UNK . \\
    \bottomrule
  \end{tabular}
  \caption{Two examples of generation.}
  \label{tab:generation}
\end{table}

==> tab-hidden-128.tex <==

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

\begin{table}
  \centering
  \begin{tabular}{llllll}
    \toprule
    Dimension & 16 & 32 & 48 & 128 & 256\\
    \midrule
    \scmh & 96.22 & 79.31 & 74.07 & 62.31 & 79.78 \\
    \scmo & 95.17 & 79.74 & 73.36 & 64.57 & 78.21 \\
    \bottomrule
  \end{tabular}
  \caption{PPL on the dev set with different hidden dimensions. The input dimension (word embedding size) is fixed as 128.}
  \label{tab:hidden-128}
\end{table}

==> tab-nant-ppl.tex <==

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

\begin{table}
  \centering
  {\footnotesize
    \begin{tabular}{llllll}
      \toprule
      & \multicolumn{2}{l}{Dimension} & & \multicolumn{2}{l}{Perplexity}\\
      \cmidrule{2-3} \cmidrule{5-6}
      Model & $K$ & $H$ & & Dev & Test\\
      \midrule
      {\em Baselines}\\
      1. RNNLM~\citep{mikolov2010recurrent} & 256 & 128 & & 109.48 & 194.43\\
      2. RNNLM w/o sentence boundary (\drnnlm) & 128 & 128 & & 101.42 & 181.62 \\
      3. Hierarchical RNNLM (\hrnnlm)~\citep{lin2015hierarchical} & 128 & 96 & & 103.90 & 175.92\\ [0.5em]
      {\em Our models}\\
      4. Attentional DCLM (\dam) & 128 & 128 & & 96.47 & {\bf 170.99}\\
      5. Context-to-output DCLM (\scmo) & 128 & 128 & & {\bf 95.10} & 173.52 \\
      6. Context-to-context DCLM (\scmh) & 256 & 96 & & 96.77 & 172.88 \\
      \bottomrule
    \end{tabular}
  }
  \caption{Perplexity on the development and test set of the North American News Text dataset.}
  \label{tab:nant-ppl}
\end{table}

==> tab-ptb-ppl.tex <==

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

\begin{table}
  \centering
  {\footnotesize
    \begin{tabular}{llllll}
      \toprule
      & \multicolumn{2}{l}{Dimension} & & \multicolumn{2}{l}{Perplexity}\\
      \cmidrule{2-3} \cmidrule{5-6}
      Model & $K$ & $H$ & & Dev & Test\\
      \midrule
      {\em Baselines}\\
      1. RNNLM~\citep{mikolov2010recurrent} & 128 & 128 & & 69.24 & 71.88\\
      2. RNNLM w/o sentence boundary (\drnnlm) & 96 & 128 & & 65.27 & 69.37\\
      3. Hierarchical RNNLM (\hrnnlm)~\citep{lin2015hierarchical} & 256 & 128 & & 66.32 & 70.62\\ [0.5em]
      {\em Our models}\\
      4. Attentional DCLM (\dam) & 128 & 96 & & 64.31 & 68.32\\
      5. Context-to-output DCLM (\scmo) & 128 & 128 & & 64.37 & 68.49\\
      6. Context-to-context DCLM (\scmh) & 128 & 128 & & {\bf 62.34} & {\bf 66.42}\\
      \bottomrule
    \end{tabular}
  }
  \caption{Perplexity on the development and test set of the Penn Treebank dataset.}
  \label{tab:ptb-ppl}
\end{table}
